Long Time Behaviour of the Two-Component Becker-D\"oring System

The classical Becker-D\"oring equations describe the formation of clusters by aggregation and fragmentation of monomers. If the total amount of mass is supercritical, larger and larger clusters are formed, leading to an asymptotic loss of mass in the long time limit. The two-component Becker-D\"oring system arises when clusters are built from two types of monomers. Here, we study the natural extension of the one-component system, where no energy or entropy is leaving or entering the system - the so called detailed balance assumption. We rigorously prove that all initial conditions admit a solution minimising the relative entropy as time approaches infinity. This shows, that the long time limit in the weak* topology is selected through the initial Type I and Type II masses. Furthermore, the proportion of lost Type I mass is determined by the limit point via the mixing ratio of Type I and Type II monomers that maximises the binding energy. The main difficulty of the two-component system is that no relative entropy is weak* continuous, which is crucial for the classical argument [2]. Instead, our proof is based on a discrete two-dimensional logarithmic Sobolev inequality, that bounds the entropy dissipation on the correct timescale. Our approach also improves current assumptions to determine the long time behaviour for the one-component system.

==> proofs/longtimeStandard.tex <==
\textbf{Step 1:} We first verify, that all the assumptions from section \ref{Preliminaries} are true. 

Since for $r+s\ge M_1$, we have $\br\rps = \ar\rs \frac{r+1}{\lambda(r+s+1)} \le \frac{\ar\rs}{\lambda}$ and $\bs\rsp = \as\rs \frac{s+1}{\mu(r+s+1} \le \frac{\as\rs}{\mu}$, we have $\ar\rs,\as\rs,\br\rps,\bs\rsp \in \mathcal O((r+s)^\alpha).$ Furthermore, we find 
\begin{equation*}
  \begin{split}
    \lim\limits_{N \to \infty} \inf\limits_{r+s \ge N} Q\rs^{\frac 1 {r+s}}
    &\ge \lim\limits_{N \to \infty} \inf\limits_{r+s \ge N} \min(\lambda,\mu) {r+s \choose r}^{\frac 1 {r+s}} e^{-(r+s)^{-\frac 1 3}}
    \ge \min(\lambda,\mu) \text{ and }\\
    \lim\limits_{N \to \infty} \sup\limits_{r+s \ge N} Q\rs^{\frac 1 {r+s}}
    &\le \lim\limits_{N \to \infty} \sup\limits_{n \ge N} \left(\sumrs[n][] Q\rs\right)^{\frac 1 {n}}
    \le \lim\limits_{N \to \infty} \sup\limits_{n \ge N} \left(\sumrs[n][] \lambda^r \mu^s {r+s \choose r}\right)^{\frac 1 {n}}\\
    &= \lim\limits_{N \to \infty} \sup\limits_{n \ge N} \left((\lambda+\mu)^n\right)^{\frac 1 {n}} = \lambda + \mu.
  \end{split}
\end{equation*}
So \eqref{assCoeff} is fulfilled.

Therefore, we can apply Theorem \ref{entropyEquation} to find that $H[c(t)|\cinfzw]$ converges monotone to some limit $H_\infty$. We want to show $H_\infty = 0$ via contradiction, so we assume that $H_\infty > 0$.

Now we fix $M_1<M<\infty$ and $\delta_1,\delta_2>0$ from Lemma \ref{relativeEntropySemicontinuity}, such that whenever $\sumrs[N+1](r+s)c\rs \le \delta_2$ is true, we already have
\[ H^\Gamma[c|\cbar] \ge \frac{H_\infty}{2} + H^\Gamma[\cbargamma(\rho^N,\sigma^N)|\cbar].\]

For an $\eps>0$, to be chosen later, we fix a time $t_1$, such that $\int_{t_1}^\infty D(c(\tau))\dd\tau < \eps.$ Furthermore, we fix $N>M,$ such that $\sumrs[\frac N 3] (r+s)c\rs(t_1) \le \frac{\delta_2} 2.$ Then, we find according to the Lemma \ref{timescale} a constant $c_{\rho_0,\sigma_0,C_a}>0$, depending only on $\rho_0,\sigma_0,C_a$, such  that
\[\sumrs[N](r+s)c\rs(t) \le \delta_2 \text{ for all } t_1\le t \le t_2 \coloneqq t_1 + c_{\rho_0,\sigma_0,C_a} N^{1-\alpha}.\]
To see this, we note that $H[c|\cinfzw]$ is uniformly bounded for all $c \in X^+_{\rho_0,\sigma_0}$ and so $\int_{t_1}^{t_2} D(c(\tau))\dd\tau \le \int_0^\infty D(c(\tau))\dd\tau \le H[c(0)|\cinfzw]\le C$. Also we have 
\[ \sup\limits_{r+s+1\ge \frac N 3} \left\{\frac {\ar\rs}{r+s}, \frac{\as\rs}{r+s}\right\}
\le C_a \sup\limits_{r+s+1\ge \frac N 3} \left\{(r+s)^{\alpha -1}\right\} \le \frac{C_a}{3^{\alpha -1}} N^{\alpha -1}.\]

\textbf{Step 2:} $D(c(t)) \ge \frac C {N^{1-\alpha}}$ for all $t\in[t_1,t_2]$ and some constant $C>0$ depending only on $H_\infty,\rho_0,\sigma_0,Q\rs,C_a,c_a$ and $\delta_1,\delta_2$.

\textbf{Step 2a:} Assume $\lambda \monr + \mu \mons \le e^{-\frac{\delta_1} 2}.$

Since $m_{n+1} = \frac{\sumrs[n+1][]\cbar\rs}{\sumrs[n][]\cbar\rs} \to \lambda \monr + \mu \mons$ with a rate independent of $\monr,\mons$, we find a constant $C_{\delta_1}$, such that $\prod\limits_{n=N_1}^{N_2} m_n \le C_{\delta_1} e^{-\frac{\delta_1}{4}(N_2-N_1 + 1)}$ for all $N_2 \ge N_1$. In particular, according to Lemma \ref{MNEstimates}, we find another constant $C_{\delta_1}$, such that 
\[ E[\Trs \cbar\kl] f\rs E\left[\Prs \frac 1 {f\kl \cbar\kl}\right] \le C_{\delta_1}.\]
From here, we can calculate
\begin{equation*}
  \begin{split}
    \frac{H_\infty}{2} + H^\Gamma[\cbargamma(\rho^N,\sigma^N)|\cbar] 
    &\le H^\Gamma[c|\cbar] 
    \le \sumrs[2][N] \cbar\rs \Psi(u\rs)\\
    \overset{\text{Theorem \ref{hardyInequality}}}&\le C_{\delta_2} \sumrs[2][N] \er\rs\cbar\rs \left(\delr \sqrt{\Psi(u\rs)}\right)^2 + \es\rs \cbar\rs \left(\dels \sqrt{\Psi(u\rs)}\right)^2\\
    &= C_{\delta_1}\Bigg[ \sumrs[2][N] \er\rps\cbar\rps \left(\delr \sqrt{\Psi(u\rps)}\right)^2 + \sumrs[2][N] \es\rsp \cbar\rsp \left(\dels \sqrt{\Psi(u\rsp)}\right)^2\Bigg]\\
    \overset{\text{Lemma \ref{erQestimate} and Remark \ref{erQEstimateAssumption}}}&\le  C_{\delta_1} \lambda \sumrs[2][N] \monr \cbar\rs \left(\delr \sqrt{\Psi(u\rps)}\right)^2 + C_{\delta_1} \mu \sumrs[2][N] \mons \cbar\rs \left(\dels \sqrt{\Psi(u\rsp)}\right)^2
  \end{split}
\end{equation*}
Finally, Lemma \ref{derivativeSqrtPsi} yields 
\begin{equation}\label{proofs:longtimeStandard:eq1}
  \begin{split}
    \frac{H_\infty}{2} + H^\Gamma[\cbargamma(\rho^N,\sigma^N)|\cbar] 
    \le C_{\delta_1} \sup\limits_{r+s \le N} \left\{ \frac{l(\max(u\rs,u\rps))}{\ar\rs}, \frac{l(\max(u\rs,u\rsp))}{\as\rs} \right\} D.
  \end{split}
\end{equation}
To understand $l(u\rs)$, we note that $u\rs = \frac{c\rs}{\cbar\rs} \le \frac{\rho_0 + \sigma_0}{\monr^r\mons^s Q\rs} \le \frac{\rho_0 + \sigma_0}{\min(\monr,\mons)^\frac 1 {r+s} Q\rs}$. So by Lemma \ref{growthL} (and \eqref{assCoeff}) we find a constant $C_{\rho_0,\sigma_0,Q\rs}$ depending only on $\rho_0,\sigma_0$ and $Q\rs$, such that 
\[ l(u\rs) \le (r+s) l\left(\frac {C_{\rho_0,\sigma_0,Q\rs}} {\min(\monr,\mons)}\right).\]
Combining \eqref{longtimeStandard:eq1} with \eqref{proofs:longtimeStandard:eq1}, we find a constant $C_{\rho_0,\sigma_0,\delta_1,\delta_2,C_a,c_a,Q\rs}$, such that 
\begin{equation*}
  \begin{split}
    \frac{1}{l\left(\frac {C_{\rho_0,\sigma_0,Q\rs}} {\min(\monr,\mons)}\right)}\left(\frac{H_\infty}{2} + H^\Gamma[\cbargamma(\rho^N,\sigma^N)|\cbar] \right)
    \le C_{\rho_0,\sigma_0,\delta_1,\delta_2,C_a,c_a,Q\rs} N^{1-\alpha} D.
  \end{split}
\end{equation*}
Finally, it remains to study the left hand side, when $\min(\monr,\mons)$ tends to zero.
To do so, we estimate 
\begin{equation*}
  \begin{split}
    H^\Gamma[\cbargamma(\rho^N,\sigma^N)|\cbar] &= \sumgamma \cbar\rs \Psi\left(\frac{\cbargamma\rs}{\cbar\rs}\right)
    = \sumgamma \cbargamma\rs\left(\ln \frac{c^\Gamma_{1,0}}{\monr} + \ln \frac{c^\Gamma_{0,1}}\mons \right) + \cbar\rs - \cbargamma\rs\\
    &\ge \rho^N \ln \frac{c^\Gamma_{1,0}}{\monr} + \sigma^N\ln \frac{c^\Gamma_{0,1}}\mons - \rho_0-\sigma_0.
  \end{split}
\end{equation*}
Now, $\rho^N$ and $\sigma^N$ are bounded away from zero. It follows, as seen in the proof of Proposition \ref{steadyStateLimit}, that $c^\Gamma_{1,0},c^\Gamma_{0,1}$ are bounded away from zero as well. So there are constants $c_{\rho_0,\sigma_0,\delta_2}$ and $C_{\rho_0,\sigma_0,\delta_2}$, such that $H^\Gamma[\cbargamma|\cbar] \ge c_{\rho_0,\sigma_0,\delta_2}\ln\left(\frac 1 {\min(\monr,\mons)}\right) - C_{\rho_0,\sigma_0,\delta_2}$. Recalling, that $l(x) = \frac{x\ln^2(x)}{4 \Psi(x)}$ and $\Psi(x) = x\ln x + 1 -x$, we see that $l(x)$ growth logarithmically for $x\to \infty.$ In particular, we find 
\[ \frac{H^\Gamma[\cbargamma|\cbar]}{l\left(\frac {C_{\rho_0,\sigma_0,Q\rs}}{\min(\monr,\mons)}\right)} \ge c_{\rho_0,\sigma_0,\delta_2,Q\rs} \text{ for }\min(\monr,\mons) \to 0.\]

\textbf{Step 2b:} Assume $\lambda\monr + \mu \mons > e^{-\frac{\delta_1} 2}$.

Let $\chat$ be constructed via \eqref{chatConstruction} and $\ccirc$ via (TODO), starting from $r+s = \max(M,M_2),$ where $M_2$ is such that
\[ e^{-(r+s)}\]


==> propositions/maxcbarLimit.tex <==
Assume \eqref{assCoeff} and \eqref{assumptionQn}. Then, $\sqrt[n]{\max\limits_{r+s = n} \cbar\rs}$ converges to $\lim\limits_{n\to\infty} q_n= q_\infty(\monr,\mons)$ for $0\le \monr,\mons$ with $\max(\monr,\mons)>0$ and the speed of convergence is independent of $\monr,\mons$, i.e. 
\[ \sqrt[n]{\max\limits_{r+s = n} \cbar\rs} = q_\infty(\monr,\mons) (1+\smallo(1))\]
and for all $\eta>0$ and any $\eps>0$, there is an $N<\infty$ , such that $|\smallo(1)| \le \eps$ for all $n\ge N$ and $\eta\le \max(\monr,\mons) \le \rho+\sigma$.

